Constrained Update Projection Approach to Safe Policy Optimization

Safe reinforcement learning (RL) studies problems where an intelligent agent has to not only maximize reward but also avoid exploring unsafe areas. In this study, we propose CUP, a novel policy optimization method based on Constrained Update Projection framework that enjoys rigorous safety guarantee. Central to our CUP development is the newly proposed surrogate functions along with the performance bound. Compared to previous safe RL methods, CUP enjoys the benefits of 1) CUP generalizes the surrogate functions to generalized advantage estimator (GAE), leading to strong empirical performance. 2) CUP unifies performance bounds, providing a better understanding and interpretability for some existing algorithms; 3) CUP provides a non-convex implementation via only first-order optimizers, which does not require any strong approximation on the convexity of the objectives. To validate our CUP method, we compared CUP against a comprehensive list of safe RL baselines on a wide range of tasks. Experiments show the effectiveness of CUP both in terms of reward and safety constraint satisfaction. We have opened the source code of CUP at this link https://github.com/zmsn-2077/ CUP-safe-rl.

==> app-related-works.tex <==
\section{Additional Discussion about Related Work}
\label{app-related-work}



This section reviews three typical safe reinforcement learning algorithms: CPO \citep{AchiamHTA17}, PCPO \citep{yang2020projection} and FOCOPS \citep{zhang2020first}.
Those algorithms also use new surrogate functions to replace the objective and constraints, which resembles the proposed CUP algorithm.
The goal is to present the contribution of our work.

\subsection{CPO \citep{AchiamHTA17}}
For a given policy $\pi_{{\bm{\theta}}_{k}}$, CPO updates new policy $\pi_{{\bm{\theta}}_{k+1}}$ as follows:
%\footnote
%{
%The objective presented by \cite{AchiamHTA17} is $\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),{\color{red}{a\sim\pi_{{\bm{\theta}}}(\cdot|s)}}}[A_{\pi_{{\bm{\theta}}_k}}(s,a)]$, which is same as the presentation in Eq.(\ref{cpo-objective}) since 
%$\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),{\color{blue}{a\sim\pi_{{\bm{\theta}}_k}(\cdot|s)}}}[\frac{\pi_{{\bm{\theta}}}(a|s)}{\pi_{{\bm{\theta}}_k}(a|s)}A_{\pi_{{\bm{\theta}}_k}}(s,a)]=\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),{\color{red}{a\sim\pi_{{\bm{\theta}}}(\cdot|s)}}}[A_{\pi_{{\bm{\theta}}_k}}(s,a)]$.
%}
\begin{flalign}
\label{app-cpo-objective}
&\pi_{{\bm{\theta}}_{k+1}}=\arg\max_{\pi_{{\bm{\theta}}}\in\Pi_{{\bm{\theta}}}}~~~~\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),a\sim\pi_{{\bm{\theta}}}(\cdot|s)}\left[A_{\pi_{{\bm{\theta}}_k}}(s,a)\right]\\
\label{app-cost-constraint}
&~~~~~~~~\text{s.t.}~~J^{c}(\pi_{{\bm{\theta}}_k})+\frac{1}{1-\gamma}\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),a\sim\pi_{{\bm{\theta}}}(\cdot|s)}\left[A^{c}_{\pi_{{\bm{\theta}}_k}}(s,a)\right]\leq b,\\
\label{app-trust-region}
&~~~~~~~~\bar{D}_{\text{KL}}(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_k})=\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot)}[\text{KL}(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_k})[s]]\leq\delta.
\end{flalign}
It is impractical to solve the problem (\ref{cpo-objective}) directly due to the computational cost.
\citep{AchiamHTA17} suggest to find some convex approximations to replace the term $A_{\pi_{{\bm{\theta}}_k}}(s,a)$ and $\bar{D}_{\text{KL}}(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_k})$ Eq.(\ref{cpo-objective})-(\ref{trust-region}).


Concretely, according to (\ref{performance-difference-2002}), \cite{AchiamHTA17} suggest to use first-order Taylor expansion of $J(\pi_{\bm{\theta}})$ to replace the objective (\ref{cpo-objective}) as follows,
\begin{flalign}
\nonumber
\frac{1}{1-\gamma}\E_{s\sim d_{\pi_{{\bm{\theta}}_k}}^{\rho_0}(\cdot),a\sim\pi_{{\bm{\theta}}_k}(\cdot|s)}\left[\dfrac{\pi_{{\bm{\theta}}}(a|s)}{\pi_{{\bm{\theta}}_k}(a|s)}A_{\pi_{{\bm{\theta}}_k}}(s,a)\right]=J(\pi_{{\bm{\theta}}})-J(\pi_{{\bm{\theta}}_k})\approx({\bm{\theta}}-{\bm{\theta}}_k)^{\top}\nabla_{{\bm{\theta}}} J(\pi_{\bm{\theta}}).
\end{flalign}
Similarly, \cite{AchiamHTA17} use the following approximations to turn the constrained policy optimization (\ref{cpo-objective})-(\ref{trust-region}) to be a convex problem,
\begin{flalign}
\label{app-contrained-01}
\frac{1}{1-\gamma}\E_{s\sim d_{\pi_{{\bm{\theta}}_k}}^{\rho_0}(\cdot),a\sim\pi_{{\bm{\theta}}_k}(\cdot|s)}&\left[\frac{\pi_{{\bm{\theta}}}(a|s)}{\pi_{{\bm{\theta}}_k}(a|s)}A^{c}_{\pi_{{\bm{\theta}}_k}}(s,a)\right]\approx({\bm{\theta}}-{\bm{\theta}}_k)^{\top}\nabla_{{\bm{\theta}}} J^{c}(\pi_{\bm{\theta}}),\\
\label{app-contrained-02}
\bar{D}_{\text{KL}}(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_k})&\approx({\bm{\theta}}-{\bm{\theta}}_k)^{\top}\mathbf{H}({\bm{\theta}}-{\bm{\theta}}_k),
\end{flalign}
where $\mathbf{H}$ is Hessian matrix of $\bar{D}_{\text{KL}}(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_k})$, i.e., 
\[\mathbf{H}[i,j]=:\dfrac{\partial^2}{\partial {\bm{\theta}}_i \partial {\bm{\theta}}_j}\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot)}\left[\text{KL}(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_k})[s]\right],\]
Eq.(\ref{app-contrained-02}) is the second-oder approximation of (\ref{trust-region}).




Let $ \lambda_{\star},\nu_{\star}$ is the dual solution of the following problem
\[
\lambda_{\star},\nu_{\star}=\arg\max_{\lambda\ge0,\nu\ge0}
\left\{
\dfrac{-1}{2\lambda}
\left(
\bg^{\top}\bH^{-1}\bg-2\nu r+sv^2
\right)
+\nu c-\dfrac{\lambda\delta}{2}
\right\}
;
\]
where
$\bg=\nabla_{\bm{\theta}}\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),a\sim\pi_{{\bm{\theta}}}(\cdot|s)}\left[A_{\pi_{{\bm{\theta}}_k}}(s,a)\right]$, $\ba=\nabla_{\bm{\theta}}\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),a\sim\pi_{{\bm{\theta}}}(\cdot|s)}\left[A^{c}_{\pi_{{\bm{\theta}}_k}}(s,a)\right]$, $r=\bg^{\top}\bH\ba,s=\ba^{\top}\bH^{-1}\ba$, and $c=J^{c}(\pi_{\bm{\theta}_k})-b$.



Finally, CPO updates parameters according to conjugate gradient as follows:
if approximation to CPO is feasible:
\begin{flalign}
\nonumber
\bm{\theta}_{k+1}=\bm{\theta}_{k}+\frac{1}{\lambda_{\star}}\bH^{-1}(\bg-\nu_{\star}\ba),
\end{flalign}
else,
\[
\bm{\theta}_{k+1}=\bm{\theta}_{k}-\sqrt{\dfrac{2\delta}{\ba^{\top}\bH^{-1}\ba}}\bH^{-1} \ba.
\]





 \subsection{PCPO \citep{yang2020projection}}
 
 
Projection-Based Constrained Policy Optimization (PCPO) is an iterative method for optimizing policies in a two-step process: the first step performs a local reward improvement update, while the second step reconciles any constraint violation by projecting the policy back onto the constraint set. 
 
 
 \textbf{Reward Improvement:}
 \begin{flalign}
 \nonumber
 \pi_{\bm{\theta}_{k+\frac{1}{2}}}=\arg\max_{\pi_{{\bm{\theta}}}\in\Pi_{{\bm{\theta}}}}\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),a\sim\pi_{{\bm{\theta}}}(\cdot|s)}\left[A_{\pi_{{\bm{\theta}}_k}}(s,a)\right],\\
 \nonumber
  \text{ s.t.} \bar{D}_{\text{KL}}(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_k})=\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot)}[\text{KL}(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_k})[s]]\leq\delta;
\end{flalign}
 \textbf{Projection:}
\begin{flalign}
\nonumber
    & \pi_{{\bm{\theta}}_{k+1}}=\arg\min_{\pi_{{\bm{\theta}}}\in\Pi_{{\bm{\theta}}}}~D\left(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_{k+\frac{1}{2}}}\right),\\
 \nonumber    
    \text{s.t.}~ J^{c}(\pi_{{\bm{\theta}}_k})&+\dfrac{1}{1-\gamma}\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),a\sim\pi_{{\bm{\theta}}}(\cdot|s)}\left[A^{c}_{\pi_{{\bm{\theta}}_k}}(s,a)\right]\leq b.
\end{flalign}


Then, \cite{yang2020projection} follows CPO \citep{AchiamHTA17} uses convex approximation to original problem, and calculate the update rule as follows,
\[
\bm{\theta}_{k+1}=\bm{\theta}_{k}-\sqrt{\dfrac{2\delta}{\bg^{\top}\bH^{-1}\bg}}\bH^{-1} \bg
-\max
\left(0,
\dfrac
{
\sqrt{\dfrac{2\delta}{\bg^{\top}\bH^{-1}\bg}}\ba^{\top}\bH^{-1} \bg+c
}
{\ba^{\top}\bL^{-1}\ba}
\right)\bL^{-1}\ba,
\]
where $\bL=\bI$ if $D$ is $\ell_2$-norm, and $\bL=\bH$ if $D$ is KL-divergence.




\subsection{FOCOPS \citep{zhang2020first}}

\cite{zhang2020first} propose the First Order Constrained Optimization in Policy Space (FOCOPS) that is a two-step approach. We present it as follows.


\textbf{Step1: Finding the optimal update policy.}
Firstly, for a given policy $\pi_{\bm{\theta}k}$, we find an optimal update policy $\pi^{\star}$ by solving the optimization problem (\ref{app-cpo-objective})-(\ref{app-trust-region}) in the non-parameterized policy space.
\begin{flalign}
\label{app-non-parameterized-01}
&\pi^{\star}=\arg\max_{\pi\in\Pi}~~~~\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),a\sim\pi(\cdot|s)}\left[A_{\pi_{{\bm{\theta}}_k}}(s,a)\right]\\
\label{app-non-parameterized-02}
&~~~~~~~~\text{s.t.}~~J^{c}(\pi_{{\bm{\theta}}_k})+\frac{1}{1-\gamma}\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),a\sim\pi(\cdot|s)}\left[A^{c}_{\pi_{{\bm{\theta}}_k}}(s,a)\right]\leq b,\\
\label{app-non-parameterized-03}
&~~~~~~~~\bar{D}_{\text{KL}}(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_k})=\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot)}[\text{KL}(\pi,\pi_{{\bm{\theta}}_k})[s]]\leq\delta.
\end{flalign}
If $\pi_{\bm{\theta}_k}$ is feasible, then the optimal policy for (\ref{app-non-parameterized-01})-(\ref{app-non-parameterized-03}) takes the following form:
\begin{flalign}
\label{optimal-solu}
\pi^{\star}(a|s)=\dfrac{\pi_{\bm{\theta}_k}(a|s)}{Z_{\lambda,\nu}(s)}\exp
\left(\dfrac{1}{\lambda}
\left(
A_{\pi_{\bm{\theta}_k}}(s,a)-\nu A^{c}_{\pi_{\bm{\theta}_k}}(s,a)
\right)
\right),
\end{flalign}
where $Z_{\lambda,\nu}(s)$ is the partition function which ensures (\ref{optimal-solu}) is a valid probability distribution, $\lambda$ and $\nu$ are solutions to the optimization problem:
\[
\min_{\lambda,\nu\ge0}\lambda\nu+\nu \tilde{b}+\lambda \E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),a\sim\pi^{\star}(\cdot|s)}\left[Z_{\lambda,\nu}(s)\right],
\]
the term $\tilde{b}=(1-\gamma)(b-J^{c}(\pi_{\bm{\theta}_k}))$.




\textbf{Step 2: Projection}
Then, we project the policy found in the previous step back into the parameterized policy space $\Pi_{\bm{\theta}}$ by solving for the closest policy $\policy\in\Pi_{\bm{\theta}}$ to $\pi^{\star}$ in order to obtain $\pi_{\bm{\theta}_{k+1}}$:
\[
\bm{\theta}_{k+1}=\arg\min_{\bm\theta} \E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot)}[\text{KL}(\pi_{{\bm{\theta}}},\pi^{\star})[s]].
\]

\subsection{Comparison to CUP}



Comparing to CPO and PCPO, the implementation of CUP does not depend on any convex approximations.
CPO learns its objective with the deep neural network via the first-order method (see Appendix \ref{sec-app-cpu}).



Concretely, CPO and PCPO approximate the non-convex objective (or constraints) with first-order or second Taylor expansion,
but their implementations still lack a theory to show the error difference between the original objective (or constraints) and its convex approximations.
Additionally, their approaches involve the inverse of a high-dimension Fisher information matrix, which causes their algorithms to require a costly computation for each update when solving high-dimensional RL problems.
While the proposed CUP does not depend on any convex approximations, it learns the policy via first-order optimization approaches.
Thus, CUP does not involve the inverse of a high-dimension Fisher information matrix, which implies CUP requires less memory than CPO and PCPO.



Although FOCOPS is also a non-convex implementation, it heavily depends on the current best-satisfied policy. 
It is known that the current best policy may not be the optimal policy, and FOCOPS requires to project this policy back into the parametric policy space, which implies FOCOPS reduce the chances for an agent to explore the environment since it may lose in a locally optimal solution.
While the proposed CUP does not depend on the current optimal policy, in fact, CUP requires the agent to learn the policy according to (\ref{performance-improvement}), the numerical solution is not the current optimal policy, which helps CUP to explore the environment.






\begin{landscape}
%\global\pdfpageattr\expandafter{\the\pdfpageattr/Rotate 90}
\renewcommand{\arraystretch}{1.5}
\begin{table}[t]
 \caption{Comparison of some safe reinforcement algorithms.}
 \label{tab:comp}
 \centering
 \small
 \setlength{\extrarowheight}{0.04cm}
 \begin{tabularx}{\linewidth}{m{2.5cm}|>{\centering}m{8cm}|>{\centering}m{7.5cm}|m{3cm}}
  \toprule
  Algorithm & Optimization problem & Implementation & Remark \\
  \midrule
  \makecell{CPO\\ \citep{AchiamHTA17}}
   & $\pi_{\bm{\theta}_{k+1}}=\arg\max_{\pi_{{\bm{\theta}}}\in\Pi_{{\bm{\theta}}}}\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),a\sim\pi_{{\bm{\theta}}}(\cdot|s)}\left[A_{\pi_{{\bm{\theta}}_k}}(s,a)\right]$,
   \newline
    s.t. $J^{c}(\pi_{{\bm{\theta}}_k})+\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),a\sim\pi_{{\bm{\theta}}}(\cdot|s)}\left[A^{c}_{\pi_{{\bm{\theta}}_k}}(s,a)\right]\leq b $,
    \newline
   $ \bar{D}_{\text{KL}}(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_k})=\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot)}[\text{KL}(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_k})[s]]\leq\delta$.
    & $\bm{\theta}_{k+1}=\arg\max_{\bm\theta}~\bg^{\top}(\bm{\theta}-\bm{\theta}_{k})$, 
    \newline
     s.t. $c+\mathbf{b}^{\top}(\bm{\theta}-\bm{\theta}_k)\leq0$,
     \newline
   $ \dfrac{1}{2}(\bm{\theta}-\bm{\theta}_k)^{\top}\mathbf{H}(\bm{\theta}-\bm{\theta}_k)\leq\delta$.
    &Convex Implementation
    \\
   \hline 
    \makecell{PCPO\\ \citep{yang2020projection}}
   &Reward Improvement $\pi_{\bm{\theta}_{k+\frac{1}{2}}}=\arg\max_{\pi_{{\bm{\theta}}}\in\Pi_{{\bm{\theta}}}}\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),a\sim\pi_{{\bm{\theta}}}(\cdot|s)}\left[A_{\pi_{{\bm{\theta}}_k}}(s,a)\right]$,
    \newline
   s.t. $\bar{D}_{\text{KL}}(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_k})=\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot)}[\text{KL}(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_k})[s]]\leq\delta$;
    \newline
    Projection
     \newline
    $\pi_{{\bm{\theta}}_{k+1}}=\arg\min_{\pi_{{\bm{\theta}}}\in\Pi_{{\bm{\theta}}}}~D\left(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_{k+\frac{1}{2}}}\right)$,
    \newline
    s.t. $J^{c}(\pi_{{\bm{\theta}}_k})+\dfrac{1}{1-\gamma}\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),a\sim\pi_{{\bm{\theta}}}(\cdot|s)}\left[A^{c}_{\pi_{{\bm{\theta}}_k}}(s,a)\right]\leq b $.
    & Reward Improvement
     \newline
    $\bm{\theta}_{k+\frac{1}{2}}=\arg\max_{\bm\theta}~\bg^{\top}(\bm{\theta}-\bm{\theta}_{k})$, 
     \newline
     s.t.$\dfrac{1}{2}(\bm{\theta}-\bm{\theta}_k)^{\top}\mathbf{H}(\bm{\theta}-\bm{\theta}_k)\leq\delta$;
    \newline
    Projection
     \newline
      $\pi_{{\bm{\theta}}_{k+1}}=\arg\min_{\bm\theta}\dfrac{1}{2}(\bm{\theta}-\bm{\theta}_k)^{\top}\mathbf{L}(\bm{\theta}-\bm{\theta}_k)$,
       \newline 
     s.t. $c+\mathbf{b}^{\top}(\bm{\theta}-\bm{\theta}_k)\leq0$.
    &Convex Implementation\\  
   \hline 
    \makecell{FOCOPS\\ \citep{zhang2020first}}
   &Optimal update policy
    \newline
    $\pi^{\star}=\arg\max_{\pi\in\Pi}\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),a\sim\pi(\cdot|s)}\left[A_{\pi_{{\bm{\theta}}_k}}(s,a)\right]$,
   \newline
    s.t. $J^{c}(\pi_{{\bm{\theta}}_k})+\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),a\sim\pi(\cdot|s)}\left[A^{c}_{\pi_{{\bm{\theta}}_k}}(s,a)\right]\leq b $,
    \newline
   $ \bar{D}_{\text{KL}}(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_k})=\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot)}[\text{KL}(\pi,\pi_{{\bm{\theta}}_k})[s]]\leq\delta$;
   \newline
   Projection
    \newline
    $\pi_{{\bm{\theta}}_{k+1}}=\arg\min_{\pi_{{\bm{\theta}}}\in\Pi_{{\bm{\theta}}}}~\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot)}[\text{KL}(\pi_{{\bm{\theta}}},\pi^{\star})[s]]$.
    & Optimal update policy
    \newline
     \newline
    $\pi^{\star}(a|s)=\frac{\pi_{\bm{\theta}_k}(a|s)}{Z_{\lambda,\nu}(s)}\exp\left(\frac{1}{\lambda}\left(A_{\pi_{\bm{\theta}_k}}(s,a)-\nu A^{c}_{\pi_{\bm{\theta}_k}}(s,a)\right)\right)$;
     \newline
      \newline
      Projection
       \newline
    $\bm{\theta}_{k+1}=\arg\min_{\bm\theta} \E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot)}[\text{KL}(\pi_{{\bm{\theta}}},\pi^{\star})[s]].$
    & Non-Convex Implementation
    \\
     \hline 
    \makecell{CUP\\ (Our Work)}
    &
    Policy Improvement
    \begin{flalign} 
    \nonumber
    \pi_{{\bm{\theta}}_{k+\frac{1}{2}}}=\arg\max_{\pi_{{\bm{\theta}}}\in\Pi_{{\bm{\theta}}}}
\bigg\{
\E_{s\sim{d}_{\pi_{\bm{\theta}_k}}^{\lambda}(\cdot),a\sim\policy(\cdot|s)}
\left[
A^{\text{GAE}(\gamma,\lambda)}_{{\pi_{\bm{\theta}_k}}}(s,a)\right]
\\
 \nonumber
-\alpha_k
\sqrt{
\E_{s\sim{d}_{{\pi_{\bm{\theta}_k}}}^{\lambda}(\cdot)}\left[\text{KL}(\pi_{\bm{\theta}_k},\policy)[s]\right]}
\bigg\},
\end{flalign}
Projection
 \begin{flalign}
\nonumber
\pi_{{\bm{\theta}}_{k+1}}=\arg\min_{\pi_{{\bm{\theta}}}\in\Pi_{{\bm{\theta}}}}~D\Big(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_{k+\frac{1}{2}}}\Big),~~~~~~~~~~~~~~~~~\\
\nonumber
 \text{s.t.} J^{c}(\pi_{{\bm{\theta}}_k})+\dfrac{1}{1-\tilde\gamma}\E_{s\sim{d}_{\pi_{\bm{\theta}_k}}^{\lambda}(\cdot),a\sim\policy(\cdot|s)}
\left[A^{\text{GAE}(\gamma,\lambda)}_{{\pi_{\bm{\theta}_k}},C}(s,a)\right]\\
\nonumber
+\beta_k\sqrt{\E_{s\sim{d}_{{\pi_{\bm{\theta}_k}}}^{\lambda}(\cdot)}\left[\text{KL}(\pi_{\bm{\theta}_k},\policy)[s]\right]}\leq b. 
\end{flalign}
    &
    Policy Improvement
     \newline
    \begin{flalign}
    \nonumber
{\bm{\theta}}_{k+\frac{1}{2}}=\arg\max_{{\bm{\theta}}}\Bigg\{\frac{1}{T}\sum_{t=1}^{T}\frac{\pi_{\bm{\theta}}(a_{t}|s_{t})}{{\pi_{\bm{\theta}_{k}}}(a_{t}|s_{t})}\hat{A}_{t}~~~~~~~~~~~~~~~~~~~~~~~~~~~~~\\
\nonumber
-\alpha\sqrt{\frac{1}{T}\sum_{t=1}^{T}\text{KL}(\pi_{\bm{\theta}_{k}}(\cdot|s_{t}),\pi_{{\bm{\theta}}}(\cdot|s_{t}))}\Bigg\};
\end{flalign}
Projection
 \newline
\begin{flalign}
\nonumber
{\bm{\theta}}_{k+1}=\arg\min_{{\bm{\theta}}} \dfrac{1}{T}\sum_{t=1}^{T}
\bigg\{
\text{KL}\left({\pi_{\bm{\theta}_{k+\frac{1}{2}}}}(\cdot|s_{t}),\pi_{{\bm{\theta}}}(\cdot|s_{t})\right)\\
\nonumber
+\nu_k
\dfrac{1-\gamma\lambda}{1-\gamma}\dfrac{\pi_{\bm{\theta}}(a_{t}|s_{t})}{\pi_{{\bm{\theta}}_k}(a_{t}|s_{t})}\hat{A}^{C}_{t}
\bigg\}.
\end{flalign}
    &
    Non-Convex Implementation
    \\
    \bottomrule
 \end{tabularx}
 \label{app-table-com}
\end{table}
\end{landscape}


==> background.tex <==

\section{Preliminaries}
\label{Background and Notations}







%\subsection{Reinforcement Learning and Policy Optimization}
Reinforcement learning (RL) \citep{sutton1998reinforcement} is often formulated as 
a \emph{Markov decision process} (MDP) \citep{puterman2014markov} that is a tuple $\mathcal{M}=(\mathcal{S},\mathcal{A},\mathbb{P},{r},\rho_0,\gamma)$.
Here $\mathcal{S}$ is state space, $\mathcal{A}$ is action space.
$\mathbb{P}(s^{'}|s,a)$ is probability of state transition from $s$ to $s^{'}$ after playing $a$.
$r(\cdot):\mathcal{S}\times\mathcal{S}\times\mathcal{A}\rightarrow \R$,
and $r(s'|s,a)$ denotes the reward that the agent observes when state transition from $s$ to $s^{'}$ after it plays $a$.
$\rho_{0}(\cdot):\mathcal{S}\rightarrow[0,1]$ is the initial state distribution and $\gamma\in(0,1)$.


A stationary parameterized policy $\policy$ is a probability distribution defined on $\mathcal{S}\times\mathcal{A}$, $\policy(a|s)$ denotes the probability of playing $a$ in state $s$.
We use $\Pi_{\bm{\theta}}$ to denote the set of all stationary policies, where $\Pi_{{{\bm{\theta}}}}=\{\pi_{{{\bm{\theta}}}}:{{\bm{\theta}}}\in\R^{p}\}$, and ${{\bm{\theta}}}$ is a parameter needed to be learned.
Let $\mathbf{P}_{\pi_{\bm \theta}}\in\R^{|\calS|\times|\calS|}$ be a state transition probability matrix, and their components are:
$
\mathbf{P}_{\pi_{\bm \theta}}[s,s'] =\sum_{a\in\mathcal{A}}\pi_{\bm{\theta}}(a|s)\mathbb{P}(s'|s,a)=:\Pro_{\policy}(s^{'}|s),
$
which denotes one-step state transformation probability from $s$ to $s^{'}$ by executing $\policy$.
Let $\tau=\{s_{t}, a_{t}, r_{t+1}\}_{t\ge0}\sim \policy$ be a trajectory generated by $\policy$, 
where $s_{0}\sim\rho_{0}(\cdot)$, $a_{t}\sim\policy(\cdot|s_t)$, $s_{t+1}\sim \mathbb{P}(\cdot|s_{t},a_{t})$, and $r_{t+1}=r(s_{t+1}|s_t,a_t)$.
We use $\mathbb{P}_{\policy}(s_t=s^{'}|s)$ to denote the probability of visiting the state $s^{'}$ after $t$
time steps from the state $s$ by executing $\policy$.
Due to the Markov property in MDP, $\mathbb{P}_{\policy}(s_t=s^{'}|s)$ is $(s,s^{'})$-th component of the matrix $\mathbf{P}^{t}_{\pi_{\bm \theta}}$, i.e.,
$
\mathbb{P}_{\policy}(s_t=s^{'}|s)=\mathbf{P}^{t}_{\pi_{\bm \theta}}[s,s^{'}].
$
Finally, let $d_{\policy}^{s_0}(s)=(1-\gamma)\sum_{t=0}^{\infty}\gamma^{t}\mathbb{P}_{\policy}(s_t=s|s_0)$ be the stationary state distribution of the Markov chain (starting at $s_0$) induced by policy $\policy$.
We define
$
d_{\policy}^{\rho_0}(s)=\mathbb{E}_{s_0\sim\rho_{0}(\cdot)}[d_{\policy}^{s_0}(s)]
$
as the discounted state visitation distribution on initial distribution $\rho_0 (\cdot)$. 



The \emph{state value function} of $\policy$ is defined as $V_{\policy}(s) = \mathbb{E}_{\policy}[\sum_{t=0}^{\infty}\gamma^{t}r_{t+1}|s_{0} = s],$
where $\mathbb{E}_{\policy}[\cdot|\cdot]$ denotes a conditional expectation on actions which are selected by $\policy$.
Its \emph{state-action value function} is $Q_{\policy}(s,a) = \mathbb{E}_{\policy}[\sum_{t=0}^{\infty}\gamma^{t}r_{t+1}|s_{0} = s,a_{0}=a]$, 
and advantage function is $A_{\policy}(s,a)=Q_{\policy}(s,a) -V_{\policy}(s)$.
The goal of reinforcement learning is to maximize $J(\policy)$:
$
  \label{J-objectiove}
  J(\policy)=\E_{s\sim d^{\rho_0}_{\policy}(\cdot)}[V_{\policy}(s)].
$





\subsection{Policy Gradient and Generalized Advantage Estimator (GAE)}

Policy gradient \citep{williams1992simple,sutton2000policy} is widely used to solve policy optimization, which maximizes the expected total reward by repeatedly estimating the gradient $g=\nabla J(\policy)$.
\cite{schulman2016high} summarize several different related expressions for the policy gradient:
\begin{flalign}
g=\nabla J(\policy)=\E\left[
\sum_{t=0}^{\infty}\Psi_{t}\nabla\log\policy(a_t|s_t)
\right],
\end{flalign}
where $\Psi_{t}$ can be total discounted reward of the trajectory, value function, advantage function or temporal difference (TD) error.
As stated by \cite{schulman2016high}, the choice $\Psi_{t}=A(s_t,a_t)$ yields almost the lowest possible variance, which is consistent with the theoretical analysis \citep{greensmith2004variance,wu2018variance}.
Furthermore, \cite{schulman2016high} propose generalized advantage estimator (GAE) $\hat{A}^{\text{GAE}(\gamma,\lambda)}_{t}(s_t,a_t)$ to replace $\Psi_{t}$: for any $\lambda\in[0,1]$,
\begin{flalign}
\hat{A}^{\text{GAE}(\gamma,\lambda)}_{t}(s_t,a_t)=\sum_{\ell=0}^{\infty}(\gamma\lambda)^{\ell}\delta^{V}_{t+\ell},
\end{flalign}
where $\delta^{V}_{t}=r_{t+1}+\gamma V(s_{t+1})-V(s_{t})$ is TD error, and $V(\cdot)$ is an estimator of value function.
GAE is an efficient technique for data efficiency and reliable performance of reinforcement learning.


\subsection{Safe Reinforcement Learning}


Safe RL \citep{Ray2019} is often formulated as 
a constrained MDP (CMDP) $\calM\cup\calC$ \citep{altman1999constrained},
which is a standard MDP $\calM$ augmented with an additional constraint set $\calC$.
The set $\calC=\{(c_i,b_i)\}_{i=1}^{m}$,
where $c_i$ are cost functions: $c_i : \calS\times\calA \rightarrow \R$, and limits are $b_i$, $i = 1,\cdot,m$. 
The \emph{cost-return} is defined as:
$J^{c_i}(\policy)=\E_{\policy}\left[\sum_{t=0}^{\infty}\gamma^{t}c_{i}(s_{t},a_{t})\right]$, 
then we define the feasible policy set $\Pi_{\calC}$ as:
$
\Pi_{\calC}=
\cap_{i=1}^{m}
\left\{
\policy\in\Pi_{\bm{\theta}}~~\text{and}~~J^{c_i}(\policy)_\leq b_i
\right\}.
$
The goal of CMDP is to search the optimal policy $\pi_{\star}$:
\begin{flalign}
\label{def:problem-setting}
\pi_{\star}=\arg\max_{\policy\in\Pi_{\calC}} J(\policy).
\end{flalign}
Furthermore, we define value functions, action-value functions, and advantage functions for the auxiliary costs in analogy to $V_{\policy}, Q_{\policy}$, and $A_{\policy}$, 
with $c_i$ replacing $r$ respectively, we denote them as $V^{c_i}_{\policy}, Q^{c_i}_{\policy}$, and $A^{c_i}_{\policy}$.
For example, $V^{c_i}_{\policy}(s) = \mathbb{E}_{\policy}\left[\sum_{t=0}^{\infty}\gamma^{t}c_i(s_{t},a_{t})|s_{0} = s\right]$.
Without loss of generality, we will restrict our discussion to the case of one constraint with a cost function $c$ and upper bound $b$.
Finally, we extend the GAE w.r.t. auxiliary cost function $c$:
\begin{flalign}
\label{def:gae-cost}
\hat{A}^{\text{GAE}(\gamma,\lambda)}_{C,t}(s_t,a_t)=\sum_{\ell=0}^{\infty}(\gamma\lambda)^{\ell}\delta^{C}_{t+\ell},
\end{flalign}
where $\delta^{C}_{t}=r_{t+1}+\gamma C(s_{t+1})-C(s_{t})$ is TD error, and $C(\cdot)$ is an estimator of cost function $c$.



\section{Generalized Policy Performance Difference Bounds}

\label{sec:generalized-bound}


In this section, we show some generalized policy optimization performance bounds for $J(\policy)$ and $J^{c}(\policy)$. 
The proposed bounds provide some new surrogate functions with respect to the objective and cost function, which are theoretical foundations for us to design efficient algorithms to improve policy performance and satisfy constraints.
Additionally, those bounds refine or extend some existing works (e.g., \citep{kakade2002approximately,schulman2015trust,AchiamHTA17}) to GAE case. Since GAE significantly
reduces variance empirically while maintains a tolerable level of bias, which is one of the key steps for us to propose efficient algorithms in the later section.




Before we present our new performance difference bounds, let us revisit a classic performance difference from \citet{kakade2002approximately},
\begin{flalign}
\label{performance-difference-2002}
J(\pi_{{\bm{\theta}}})-J(\policyy)
=(1-\gamma)^{-1}\E_{s\sim d_{\policy}^{\rho_0}(\cdot),a\sim\policy (\cdot|s)}\left[A_{\policyy}(s,a)\right].
\end{flalign}
Eq.(\ref{performance-difference-2002}) shows a difference between two arbitrary policies $\pi_{\bm\theta}$ and $\pi_{{\bm\theta}^{'}}$ with different parameters $\bm{\theta}$ and $\bm{\theta}^{'}$.
According to (\ref{performance-difference-2002}), we rewrite the policy optimization (\ref{def:problem-setting}) as follows
\begin{flalign}
\label{def:rewriting-problem-setting}
\pi_{\star}=\arg\max_{\policy\in\Pi_{\calC}} \E_{s\sim d_{\policy}^{\rho_0}(\cdot),a\sim\policy (\cdot|s)}\left[A_{\policyy}(s,a)\right].
\end{flalign}
However, Eq.(\ref{performance-difference-2002}) or (\ref{def:rewriting-problem-setting}) is very intractable for sampling-based policy optimization since it requires the data comes from the (unknown) policy $\policy$ that needed to be learned.


In this section, our new bound refines the result (\ref{performance-difference-2002}), which provide the sights for surrogate functions to solve safe RL problem (\ref{def:problem-setting}).
For more discussions about the difference between our new bound and Eq.(\ref{performance-difference-2002}), see Remark \ref{remark:Comparison-with-kakade}.

\clearpage




In this section, we show some generalized policy optimization performance bounds for $J(\policy)$ and $J^{c}(\policy)$. 
The proposed bounds provide some new certain surrogate functions w.r.t. the objective and cost function, which are theoretical foundations for us to design efficient algorithms to improve policy performance and satisfy constraints.
Additionally, those bounds refine or extend some existing works (e.g., \citep{kakade2002approximately,schulman2015trust,AchiamHTA17}) to GAE case that significantly
reduces variance while maintains a tolerable level of bias, which is one of the key steps for us to propose efficient algorithms in the later section.




Before we present our new bounds, let us revisit a classic result about policy performance difference from \citep{kakade2002approximately}, i.e., the next Eq.(\ref{performance-difference-2002}),
\begin{flalign}
\label{performance-difference-2002}
J(\pi_{{\bm{\theta}}})-J(\policyy)
=(1-\gamma)^{-1}\E_{s\sim d_{\policy}^{\rho_0}(\cdot)}\E_{a\sim\policy (\cdot|s)}[A_{\policyy}(s,a)].
\end{flalign}
Eq.(\ref{performance-difference-2002}) shows a difference between two arbitrary policies $\pi_{\bm\theta}$ and $\pi_{{\bm\theta}^{'}}$ with different parameters $\bm{\theta}$ and $\bm{\theta}^{'}$.
However, as stated by \cite{zanger2021safe}, Eq.(\ref{performance-difference-2002}) is very intractable for sampling-based policy optimization since it requires the data comes from a fixed policy $\policy$.
In this section, our new bound will refine the result (\ref{performance-difference-2002}). For more discussions about the difference between our new bound and Eq.(\ref{performance-difference-2002}), please refer to Remark \ref{remark:Comparison-with-kakade}.



   
\subsection{Some Additional Notations}



We use a bold lowercase letter to denote a vector, e.g., $\ba=(a_1,a_2,\cdots,a_n)$, and its $i$-th element $\ba[i]=:a_{i}$.
Let $\varphi(\cdot):\calS\rightarrow\R$ be a function defined on $\calS$, $\delta_t^{\varphi}=r(s_{t+1}|s_t,a_t)+\gamma\varphi(s_{t+1})-\varphi(s_{t})$ is TD error w.r.t. $\varphi(\cdot)$. 
For two arbitrary policies $\pi_{\bm\theta}$ and $\pi_{{\bm\theta}^{'}}$, we denote $\delta^{\varphi}_{\policy,t}(s)$ as the expectation of TD error, and define $ \Delta_{t}^{\varphi}(\policy,\policyy,s)$ as the difference between $\delta^{\varphi}_{\policy,t}(s)$ and $\delta^{\varphi}_{\policyy,t}(s)$: $\forall s\in\calS$, 
\begin{flalign}
\nonumber
\delta^{\varphi}_{\policy,t}(s)=\underset{\begin{subarray}{c} s_t \sim \Pro_{\policy}(\cdot|s)\\ a_{t}\sim{\policy}(\cdot|s_t)\\ s_{t+1}\sim\Pro(\cdot|s_t,a_t) \end{subarray}}\E\left[\delta_t^{\varphi}\right],
\Delta_{t}^{\varphi}(\policy,\policyy,s)=
\underset{\begin{subarray}{c} s_t \sim \Pro_{\policyy}(\cdot|s)\\ a_{t}\sim{\policyy}(\cdot|s_t)\\ s_{t+1}\sim\Pro(\cdot|s_t,a_t) \end{subarray}}
\E\left[\left(\dfrac{\policy(a_t|s_t)}{\policyy(a_t|s_t)}-1\right)\delta_t^{\varphi}\right].
\end{flalign}
Furthermore, we introduce two vectors $\bm{\delta}^{\varphi}_{\policy,t},\bm{\Delta}_{t}^{\varphi}(\policy,\policyy)\in\R^{|\calS|}$, and their components are:
\begin{flalign}
\bm{\delta}^{\varphi}_{\policy,t}[s]=\delta^{\varphi}_{\policy,t}(s),~~~\bm{\Delta}_{t}^{\varphi}(\policy,\policyy)[s]=\Delta_{t}^{\varphi}(\policy,\policyy,s).
\end{flalign}
Let matrix $\mathbf{P}^{(\lambda)}_{\pi_{\bm \theta}}=(1-\gamma\lambda)\sum_{{t}=0}^{\infty}(\gamma\lambda)^{{t}}\bP^{{t}+1}_{\policy}$, 
where $\lambda\in[0,1]$.
%and its $(s,s^{'})$-th component denoted as$\Pro_{\policy}^{(\lambda)}(s^{'}|s)=:\mathbf{P}^{(\lambda)}_{\pi_{\bm \theta}}[s,s^{'}].$
It is similar to the normalized discounted distribution $d_{\pi_{\bm {\theta}}}^{\rho_0}(s)$, we extend it to $\lambda$-version and denote it as ${d}_{\pi_{\bm {\theta}}}^{\lambda}(s)$:
\[
{d}_{\pi_{\bm {\theta}}}^{\lambda}(s)=\E_{s_0\sim\rho_{0}(\cdot)}
\left[
(1-\tilde\gamma)\sum_{t=0}^{\infty}{\tilde\gamma}^{t}{\mathbb{P}}^{(\lambda)}_{\pi_{\bm {\theta}}}(s_t=s|s_0)
\right],
\]
where $\tilde{\gamma}=\frac{\gamma(1-\lambda)}{1-\gamma\lambda}$, the probability $\mathbb{P}^{(\lambda)}_{\pi_{\bm {\theta}}}(s_t=s|s_0)$ is the $(s_0,s)$-th component of the matrix product $\left(\mathbf{P}^{(\lambda)}_{\pi_{\bm \theta}}\right)^{t}$.
Finally, we introduce a vector $\bd_{\pi_{\bm {\theta}}}^{\lambda}\in\R^{|\calS|}$, and its components are: $\bd_{\pi_{\bm {\theta}}}^{\lambda}[s]=d_{\pi_{\bm {\theta}}}^{\lambda}(s).$

\subsection{Main Results}

\begin{theorem}
[Generalized Policy Performance Difference]
\label{them:general-performance-difference}
For any function $\varphi(\cdot):\calS\rightarrow\R$, for two arbitrary policies $\pi_{\bm\theta}$ and $\pi_{{\bm\theta}^{'}}$,  
for any $p,q\in[1,\infty)$ such that $\frac{1}{p}+\frac{1}{q}=1$, we define two error terms:
\begin{flalign}
\label{error-01}
&\epsilon^{\varphi,(\lambda)}_{p,q,t}(\policy,\policyy)=:\|\bd_{\pi_{\bm {\theta}}}^{\lambda}-\bd_{\policyy}^{\lambda}\|_{p}\|{\bm{\delta}}^{\varphi}_{\policy,t}\|_{q},\\
\label{error-02}
L^{\varphi, \pm}_{p,q}(\policy,\policyy)&=:
\dfrac{1}{1-\tilde\gamma}
\sum_{t=0}^{\infty}\gamma^t\lambda^{t}\E_{s\sim{d}_{\policyy}^{\lambda}(\cdot)} \left[
\Delta_{t}^{\varphi}(\policy,\policyy,s) \pm\epsilon^{\varphi,(\lambda)}_{p,q,t}(\policy,\policyy)\right].
\end{flalign}
Then, the following bound w.r.t. policy performance difference $J(\pi_{\bm \theta})-J(\pi_{{\bm \theta}^{'}})$ holds:
\begin{flalign} 
\label{bound-diff-01}
L^{\varphi,-}_{p,q,}(\policy,\policyy)
\leq J(\pi_{\bm \theta})-J(\pi_{{\bm \theta}^{'}})
\leq
L^{\varphi,+}_{p,q,}(\policy,\policyy)
.
\end{flalign}
\end{theorem}
\begin{proof}
See Appendix \ref{sec:proof-them-01}.
\end{proof}
The bound (\ref{bound-diff-01}) is \emph{tight}, i.e., if $\policy=\policyy$, all the three terms in Eq.(\ref{bound-diff-01}) are zero identically.
From Eq.(\ref{error-02}), we know the performance difference bound
$L^{\varphi, \pm}_{p,q}(\policy,\policyy)$ (\ref{bound-diff-01}) can be interpreted by two distinct difference parts:
\textbf{(i)} the first difference part, i.e., the expectation $\Delta_{t}^{\varphi}(\policy,\policyy,s)$, which is determined by the difference between TD errors of $\policy$ and $\policyy$;
\textbf{(ii)} the second difference part, i.e., the discounted distribution difference $\epsilon^{\varphi,(\lambda)}_{p,q,t}(\policy,\policyy)$, which is determined by the gap between the normalized discounted distribution of $\policy$ and $\policyy$.
Thus, the difference of both TD errors and discounted distribution determine the policy difference $J(\policy)-J(\policyy)$.


The different choices of $p$ and $q$ lead Eq.(\ref{bound-diff-01}) to be different bounds.
If $p=1,q=\infty$, we denote $\epsilon^{\varphi}_{\policy,t}=:\|{\bm{\delta}}^{\varphi}_{\policy,t}\|_{q}=\max_{s_{t}\in\calS}\E_{a_t\sim\policy(\cdot|s_t),s_{t+1}\sim\Pro(\cdot|s_t,a_t)}[|\delta_{t}^{\varphi}|]$,
then,
according to Lemma \ref{lem:difference-distri} (see Appendix \ref{sec:difference-distri}), when $p=1,q=\infty$, then error $\epsilon^{\varphi,(\lambda)}_{p,q,t}(\policy,\policyy)$ is reduced to:
\begin{flalign}
\nonumber
\epsilon^{\varphi,(\lambda)}_{p,q,t}(\policy,\policyy)\big|_{p=1,q=\infty}
\leq\dfrac{1}{1-\tilde\gamma}\cdot
\dfrac{\gamma(1-\lambda)\epsilon^{\varphi}_{\policy,t}}{\left|1-2\gamma\lambda|\calS||\calA|\right|}
\E_{s\sim d_{\policyy}^{\lambda}(\cdot)}
\left[2D_{\text{TV}}(\policyy,\policy)[s]\right],
\end{flalign}
where $D_{\text{TV}}(\policyy,\policy)[s]$ is the total variational divergence between action distributions at state $s$, i.e.,
\[
2D_{\text{TV}}(\policyy,\policy)[s]=\sum_{a\in\calA}\left|{{\policyy}}(a|s)-{{\policy}}(a|s)\right|.
\]
Finally, let $\varphi=V_{\policyy}$, the left side of (\ref{bound-diff-01}) in Theorem \ref{them:general-performance-difference} implies a lower bound of performance difference, which illustrates the worse case of approximation error, we present it in Proposition \ref{propo-01}.
\begin{proposition}[Worse case approximation error]
\label{propo-01}
For any two policies $\pi_{\bm\theta}$ and $\pi_{{\bm\theta}^{'}}$, let $\epsilon^{V}_{\policy}(\policyy)=:\sup_{t\in\N^{+}}\{\epsilon^{\varphi}_{\policy,t}: \varphi=V_{\policyy}\}$, then the following bound holds
\begin{flalign}
\label{pro1-bound-01}
&J(\policy)-J(\policyy)\\
\ge&
\nonumber
\frac{1}{1-\tilde\gamma}\E_{s\sim{d}_{\policyy}^{\lambda}(\cdot),a\sim\policy(\cdot|s)}
\left[
A^{\emph{GAE}(\gamma,\lambda)}_{\policyy}(s,a)
-
\frac{2\gamma(1-\lambda)\epsilon^{V}_{\policy}(\policyy)}{(1-\gamma\lambda)\left|1-2\gamma\lambda|\calS||\calA|\right|}
D_{\emph{TV}}(\policyy,\policy)[s]
\right].
\end{flalign}
\end{proposition}
If $\lambda\rightarrow0$, then the distribution ${d}_{\policyy}^{\lambda}(\cdot)$ is reduced to ${d}_{\policyy}^{\rho_0}(\cdot)$ and the bound (\ref{pro1-bound-01}) is reduced to 
\begin{flalign}
\label{bound-lam-0}
J(\policy)-J(\policyy)
\ge
\frac{1}{1-\gamma}\E_{s\sim{d}_{\policyy}^{\rho_0}(\cdot),a\sim\policy(\cdot|s)}
\left[
A_{\policyy}(s,a)
-2\gamma\epsilon^{V}_{\policy}(\policyy)
D_{\text{TV}}(\policyy,\policy)[s]
\right].
\end{flalign}
Let us review \citep[Corollary 1]{AchiamHTA17}, which shows 
\begin{flalign}
\label{bound-achiam17-icml}
J(\policy)-J(\policyy)
\ge
\frac{1}{1-\gamma}\E_{s\sim{d}_{\policyy}^{\rho_0}(\cdot),a\sim\policy(\cdot|s)}
\left[
A_{\policyy}(s,a)
-2\frac{\gamma\epsilon^{V}_{\policy}(\policyy)}{1-\gamma}
D_{\text{TV}}(\policyy,\policy)[s]
\right].
\end{flalign}
Comparing (\ref{bound-lam-0}) to (\ref{bound-achiam17-icml}), our new bound (\ref{bound-lam-0}) is slightly tighter than the bound shown by \citep{AchiamHTA17}, concretely, our result improves the bound (\ref{bound-achiam17-icml}) by a factor $\frac{1}{1-\gamma}$.
The bound (\ref{bound-achiam17-icml}) has been used as a surrogate function for $J(\policy)-J(\policyy)$, and this idea has been developed as \emph{constrained policy optimization} by extensive works (e.g., \citep{koller2018learning,zhang2020first,yang2020accelerating,yang2020projection,zanger2021safe}).
%In the later section, we will develop our refined bound (\ref{pro1-bound-01}) as a new surrogate function. 
Since the refined bound (\ref{pro1-bound-01}) contains GAE technique that significantly reduces variance while maintains a tolerable level of bias \citep{schulman2016high}, which implies using the bound (\ref{pro1-bound-01}) as a surrogate function could improve performance potentially.


\begin{remark}[Comparison with \citep{kakade2002approximately}]
\label{remark:Comparison-with-kakade}
The result (\ref{pro1-bound-01}) develops the classic performance difference (\ref{performance-difference-2002}) at least two aspects.
Firstly, the bound (\ref{pro1-bound-01}) extends from the advantage $A_{\policyy}$ (\ref{performance-difference-2002}) to GAE function $A_{\policyy}^{\emph{GAE}(\gamma,\lambda)}$.
Secondly, the following term in Eq.(\ref{pro1-bound-01}):
\begin{flalign}
\label{gap-01}
\dfrac{1}{1-\tilde\gamma}\E_{s\sim{d}_{\policyy}^{\lambda}(\cdot),a\sim\policy(\cdot|s)}\left[A^{\emph{GAE}(\gamma,\lambda)}_{\policyy}(s,a)\right]
\end{flalign} 
is an approximation for the difference $J(\policy)-J(\policyy)$,
while Eq.(\ref{performance-difference-2002}) shows an identity for difference $J(\policy)-J(\policyy)$.
It seems that Eq.(\ref{performance-difference-2002}) is a natural objective for return maximization, however, Eq.(\ref{performance-difference-2002}) is very intractable for sampling-based policy optimization since Eq.(\ref{performance-difference-2002}) requires the data comes from a fixed policy $\policy$ \citep{zanger2021safe}.
The approximation (\ref{gap-01}) solves this problem by the expectation over the state distribution $d_{\policyy}^{\lambda}(\cdot)$ w.r.t. policy $\policyy$ and action distribution of another policy $\policy$.
Thus, bound (\ref{pro1-bound-01}) provides a tractable objective for sample-based optimization.
\end{remark}












Let $\varphi=V^{c}_{\policyy}$, Theorem \ref{them:general-performance-difference} implies an upper bound of cost function as presented in the next Proposition \ref{pro-02}, we will use it to make guarantee for safe policy optimization.

\begin{proposition}
\label{pro-02}
For any two policies $\pi_{\bm\theta}$ and $\pi_{{\bm\theta}^{'}}$, let $\epsilon^{C}_{\policy}(\policyy)=:\sup_{t\in\N^{+}}\{\epsilon^{\varphi}_{\policy,t}: \varphi=V^{c}_{\policyy}\}$, then
% the following bound holds
\begin{flalign}
\label{pro2-bound-02}
&J^{c}(\policy)-J^{c}(\policyy)\\
\leq&
\nonumber
\dfrac{1}{1-\tilde\gamma}\E_{s\sim{d}_{\policyy}^{\lambda}(\cdot),a\sim\policy(\cdot|s)}
\left[
A^{\emph{GAE}(\gamma,\lambda)}_{\policyy,C}(s,a)
+
\frac{2\gamma(1-\lambda)\epsilon^{C}_{\policy}(\policyy)}{(1-\gamma\lambda)\left|1-2\gamma\lambda|\calS||\calA|\right|}
D_{\emph{TV}}(\policyy,\policy)[s]
\right],
\end{flalign}
where we calculate $A^{\emph{GAE}(\gamma,\lambda)}_{\policyy,C}(s,a)$ according to the data sampled from $\policyy$ and (\ref{def:gae-cost}).
\end{proposition}



All above bound results (\ref{pro1-bound-01}) and (\ref{pro2-bound-02}) can be extended for a total variational divergence to KL-divergence between policies, which are desirable for policy optimization.
We obtain
\begin{flalign}
\label{inequlities}
\E_{s\sim{d}_{\policyy}^{\lambda}(\cdot)}\left[D_{\text{TV}}(\policyy,\policy)[s]\right]
\leq&
\E_{s\sim{d}_{\policyy}^{\lambda}(\cdot)}\left[\sqrt{\frac{1}{2}\text{KL}(\policyy,\policy)[s]}\right]
\leq
\sqrt{\frac{1}{2}\E_{s\sim{d}_{\policyy}^{\lambda}(\cdot)}\left[\text{KL}(\policyy,\policy)[s]\right]},
\end{flalign}
where $\text{KL}(\cdot,\cdot)$ is KL-divergence, and $\text{KL}(\policyy,\policy)[s]=\text{KL}(\policyy(\cdot|s),\policy(\cdot|s))$; the first inequality follows Pinsker's inequality \citep{csiszar2011information} and the second inequality follows Jensen's inequality.
According to (\ref{inequlities}), we obtain the next Proposition \ref{propo-03}.
\begin{proposition}
\label{propo-03}
All the bounds in (\ref{pro1-bound-01}) and (\ref{pro2-bound-02}) hold if we make the following substitution:
\[
\E_{s\sim{d}_{\policyy}^{\lambda}(\cdot)}\left[D_{\emph{TV}}(\policyy,\policy)[s]\right]
\leftarrow
\sqrt{\frac{1}{2}\E_{s\sim{d}_{\policyy}^{\lambda}(\cdot)}\left[\emph{KL}(\policyy,\policy)[s]\right]}.
\]
\end{proposition}
















==> experiment.tex <==
\begin{figure*}[t!]
 \centering
 \subfigure[Walker2d-v3]
{\includegraphics[width=3.4cm,height=2.5cm]{final_fig/Walker2d_prefinal.pdf}}
\subfigure[Walker2d-v3]
{\includegraphics[width=3.4cm,height=2.5cm]{final_fig/Walker2d_prefinal_cost.pdf}}
\subfigure[Hopper-v3]
{\includegraphics[width=3.4cm,height=2.5cm]{final_fig/Hopper_prefinal.pdf}}
\subfigure[Hopper-v3]
{\includegraphics[width=3.4cm,height=2.5cm]{final_fig/Hopper_prefinal_cost.pdf}}
 \caption{
 Learning curves for reward and cost on robots with speed limit tasks. 
 }
\label{fig-1}
\end{figure*}
\begin{figure*}[t!]
 \centering
 \subfigure[AntCircle-v0]
{\includegraphics[width=3.4cm,height=2.5cm]{final_fig/ant_circle_prefinal.pdf}}
\subfigure[AntCircle-v0]
{\includegraphics[width=3.4cm,height=2.5cm]{final_fig/ant_circle_prefinal_cost.pdf}}
\subfigure[HumanoidCircle-v0]
{\includegraphics[width=3.4cm,height=2.5cm]{final_fig/human_circle_pre_final.pdf}}
\subfigure[HumanoidCircle-v0]
{\includegraphics[width=3.4cm,height=2.5cm]{final_fig/human_circle_pre_final_cost.pdf}}
 \caption{
  Learning curves for reward and cost on circle tasks. 
 }
\label{fig-2}
\end{figure*}


\section{Experiments}



In this section, we show the effectiveness of CUP on three different sets of experiments (including seven tasks):
(i) robots with speed limit \citep{zhang2020first}; (ii) circle task \citep{AchiamHTA17}; (iii) robot options and desiderata \citep{Ray2019}.


For task (i), we train different robotic agents to move along a straight line or a two-dimensional plane, but the robot's speed is constrained for safety purposes.
For task (ii), the agent is rewarded for running in a wide circle but is constrained to stay within a safe region smaller than the radius of the target circle.
Task (iii) is safety Gym ships with three pre-made robots that we use in the benchmark environments from \citep{Ray2019}.
All of those details are provided in Appendix \ref{sec:app-ex-env}.

\textbf{Baseline algorithms}.
We compare CUP to CPO \citep{AchiamHTA17}, PCPO-KL \citep{yang2020projection}, FOCOPS \citep{zhang2020first} in the task (i) and task (ii).
To make a more comprehensive comparison, we compare CUP with the unconstrained algorithms TRPO \citep{schulman2015trust} and PPO \citep{schulman2017proximal}, and compare CUP with two additional safe RL algorithms TRPO-Lagrangian and PPO-Lagrangian, that combine the Lagrangian approach with TRPO and PPO.


\begin{table}[t]
  \centering
  \caption{Bootstrap mean with 100 bootstrap samples of reward/cost return after training on robot with speed limit environments. Cost thresholds are in brackets under the environment names.}
  % \begin{footnotesize}
  \vskip 0.1in
  \begin{adjustbox}{width=\textwidth}
  \begin{tabular}{*6c}
  \toprule
  Environment  & {} & FOCOPS & CPO & PCPO & \textbf{CUP} \\
  \midrule
  Walker2d-v3 &Reward & $1798.1\pm 0.3$ & $1076.9\pm 9.8$ & $1039.5\pm 5.2$ & $\boldsymbol{2964.3\pm 10.8}$ \\
  (82) &Cost & $82.3\pm 0.03$ & $107.82\pm 1.16$ & $100.25\pm 0.67$ & $73.9\pm 0.09$ \\
  \midrule
  Hopper-v3 &Reward & $1869.3\pm 2.8$ & $1056.0\pm 5.0$ & $1071.1\pm 4.6$ & $\boldsymbol{2409.8\pm 5.6}$ \\
  (82) &Cost & $83.1\pm 0.1$ & $90.0\pm 8.2$ & $74.8\pm 8.2$ & $80.0\pm 0.1$ \\
  \midrule
  AntCircle-v0 &Reward & $1206.3\pm 159.1$ & $423.3\pm 12.6$ & $342.9\pm 5.5$ & $\boldsymbol{1879.7\pm 79.4}$ \\
  (50) &Cost & $44.1\pm 4.2$ & $51.3\pm 1.5$ & $51.2\pm 2.4$ & $49.3\pm 2.0$ \\
    \midrule
  HumanoidCircle-v0 &Reward & $963.0\pm 40.0$ & $329.5\pm 1.7$ & $244.5\pm 7.5$ & $\boldsymbol{1029\pm 49.0}$ \\
  (50) &Cost & $50.6\pm 1.9$ & $46.0\pm 0.4$ & $47.1\pm 1.3$ & $48.4\pm 2.8$ \\
  \bottomrule
  \end{tabular}
  \end{adjustbox}
  \label{tab:mujoco_velocity_results}
  % \end{footnotesize}
\end{table}
\begin{table}[t]
  \centering
  \caption{Normalized metrics from the conclusion of training averaged over various slates of environments and three random seeds per environment. The data of PPO,PPO-L,TRPO,and TRPO-L are same to \citep{Ray2019}}
  % \begin{footnotesize}
  \vskip 0.1in
  \begin{adjustbox}{width=\textwidth}
  \begin{tabular}{cccc|cccc|cccc}
  \toprule
  SGPoint & $\bar{J}_r$ &$ \bar{M}_c$ & $\bar{\rho}_c$ & SGCar&$\bar{J}_r$&$ \bar{M}_c$ &$\bar{\rho}_c$&SGDoggo&$\bar{J}_r$&$ \bar{M}_c$&$\bar{\rho}_c$\\
  \midrule
  PPO & $1.0$ & $1.0$ & $1.0$ & &$1.0$&$1.0$&$1.0$&&$1.0$&$1.0$&$1.0$\\
  \midrule
  PPO-L & $0.348$ & $0.504$ & $0.278$ & &$0.373$&$\boldsymbol{0.004}$&$0.238$&&$0.0$&$0.021$&$0.218$\\
    \midrule
  TRPO & $1.436$ & $0.975$ & $0.967$ & &$1.158$&$0.909$&$1.017$&&$0.688$&$1.513$&$1.029$\\
   \midrule
  TRPO-L & $0.565$ & $0.014$ & $\boldsymbol{0.274}$ & &$0.374$&$0.022$&$0.244$&&$0.054$&$0.019$&$0.277$\\
   \midrule
  CPO & $1.005$ & $0.353$ & $0.514$ & &$0.794$&$0.361$&$0.545$&&$0.552$&$1.065$&$0.878$\\
  \midrule
  PCPO & $1.017$ & $0.233$ & $0.294$ & &$1.072$&$0.051$&$0.651$&&$0.884$&$0.853$&$0.533$\\
  \midrule
  CUP & $\boldsymbol{1.501}$ & $\boldsymbol{0.013}$ & $0.285$ & &$\boldsymbol{1.472}$&$0.031$&$\boldsymbol{0.229}$&&$\boldsymbol{1.096}$&$\boldsymbol{0.007}$&$\boldsymbol{0.214}$\\
  \bottomrule
  \end{tabular}
  \end{adjustbox}
  \label{tab:safr-gym-results}
  % \end{footnotesize}
\end{table}






\subsection{Robots with Speed Limit and circle task}


Figure \ref{fig-1}-\ref{fig-2} show the earning curves for robots with speed limit tasks and circle tasks, where the x-axis represents the iteration number, and the y-axis represents the average total reward/cost return of the last 100 episodes. The solid line represents the mean of last 100 episodes, and the shaded regions represent the variance of those 100 samples.


Figure \ref{fig-1}-\ref{fig-2} show that both CUP and FOCOPS consistently enforce approximate constraint satisfaction while CUP has a higher performance than FOCOPS.
CUP outperforms CPO and PCPO significantly for both reward and cost.
Those observations suggest the projection step of CUP helps the agent to learn the safe constraints.
We notice PCPO also has a projection step, CUP performs better than PCPO due to CUP learning the objective and constraints under a non-convex function while PCPO uses its convex approximation, which is one motivation for us to propose CUP.



\subsection{Safety Gym Ships with Three Pre-made Robots}

\label{three-pre-made-robots}

We compare the algorithms on three environments SGPoint, SGCar, and SGDoggo, which are all six Point/Car/Doggo robot environments with constraints in Safety Gym.
Thus, it is necessary to introduce the rule for comparing the aggregate performance of algorithms across many environments by \citep{Ray2019}, where it assigns each environment $\mathcal{E}$ a set of characteristic metrics, $\bar{J}^{\calE}_r$, $\bar{J}^{\calE}_c$, $\bar{\rho}^{\calE}_c$ and
compute normalized return $\bar{J}_r$, normalized constraint violation $ \bar{M}_c$, and normalized cost rate $\bar{\rho}_c$:
\[
\bar{J}_r=\dfrac{J(\policy)}{\bar{J}^{\calE}_r}, ~ \bar{M}_c=\dfrac{\max\{0,J_c(\policy)-d\}}{\max\{10^{-6},\bar{J}^{\calE}_c-d\}},~\bar{\rho}_c=\dfrac{\bar{\rho}_c}{\bar{\rho}^{\calE}_c}.
\]


We have provided all the details of hyper-parameters in Appendix \ref{sec:app-ex}.
In Table \ref{tab:safr-gym-results}, we show the normalized metrics from the conclusion of training averaged over various slates of environments and three random seeds per environment.
Results show that cost and rewards trade off happens in SGPoint and SGCar, while CUP achieves the best performance in those two environments.
In the SGDoggo environment, CUP achieves the best performance and constraint satisfaction over all the baseline algorithms.


\section{Conclusion}
In this paper, we propose the CUP algorithm with a theoretical safety guarantee.
We derive the CUP bases on some new proposed surrogate functions w.r.t. objective and constraints and the practical implementation of CUP does not depend on any convex approximation.
Extensive experiments on continuous control tasks show the effectiveness of CUP where the agent satisfies safe constraints.






==> method.tex <==
\section{CUP: Conservative Update Policy}
\label{sec:algorithm}



%It is challenging to implement CMDP (\ref{def:problem-setting}) directly since it requires us to judge whether a proposed policy $\policy$ is in the feasible region $\Pi_{\calC}$.
According to the bounds in Proposition \ref{propo-01}-\ref{propo-03}, we develop new surrogate functions to replace the objective and constraints.
%Inspired by two recent works \citep{yang2020projection,zhang2020first}, 
We propose the CUP (conservative update policy) algorithm that is a two-step approach contains \emph{performance improvement} and \emph{projection}.
Theorem \ref{them-re-cost} shows the proposed CUP guarantees the policy improvement and safety constraints.




\textbf{Step 1: Performance Improvement.}


According to Proposition \ref{propo-01} and Proposition \ref{propo-03}, for an appropriate coefficient $\alpha_k$, we update policy as:
\begin{flalign}
\label{performance-improvement}
\pi_{{\bm{\theta}}_{k+\frac{1}{2}}}&=\arg\max_{\pi_{{\bm{\theta}}}\in\Pi_{{\bm{\theta}}}}
\left\{
\underset{\begin{subarray}{c}s \sim{d}_{\pi_{\bm{\theta}_k}}^{\lambda}(\cdot)\\a\sim\pi_{\bm{\theta}_k}(\cdot|s)\end{subarray}}
\E\left[\frac{\pi_{\bm{\theta}}(a|s)}{\pi_{{\bm{\theta}}_k}(a|s)}
A^{\text{GAE}(\gamma,\lambda)}_{{\pi_{\bm{\theta}_k}}}(s,a)\right]-\alpha_k
\sqrt{
\E_{s\sim{d}_{{\pi_{\bm{\theta}_k}}}^{\lambda}(\cdot)}\left[\text{KL}(\pi_{\bm{\theta}_k},\policy)[s]\right]}
\right\},
\end{flalign}
%This step is a typical minimization-maximization (MM) algorithm \citep{hunter2004tutorial}, it includes return maximization and minimization the distance between old policy and new policy.
%This idea has appeared in \citep{schulman2015trust} that is guaranteed to produce policies with monotonically improvement, and we extend this idea to GAE.
We replace (\ref{performance-improvement-01}) with an importance sampling with respect to $\pi_{\bm{\theta}_k}$ to obtain the expectation (\ref{performance-improvement}), and all the remains is to replace the expectation (\ref{performance-improvement}) by sample averages according to the trajectories collected by $\pi_{\bm{\theta}_k}$.



\textbf{Step 2: Projection.}


According to Proposition \ref{pro-02} and Proposition \ref{propo-03}, for an appropriate coefficient $\beta_k$, we project the policy $\pi_{{\bm{\theta}}_{k+\frac{1}{2}}}$ onto the safe constraint set.
Concretely, we use a measure $D(\cdot,\cdot)$ (e.g., KL divergence or $\ell_2$-norm) to minimize distance between $\pi_{{\bm{\theta}}_{k+\frac{1}{2}}}$ and $\policy$, and require the new policy satisfies the safe constraint:
\begin{flalign}
\label{projection}
&~~~~~~~~~~~~~~~~~\pi_{{\bm{\theta}}_{k+1}}=\arg\min_{\pi_{{\bm{\theta}}}\in\Pi_{{\bm{\theta}}}}~D\left(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_{k+\frac{1}{2}}}\right),\\
\nonumber
&\text{s.t.}~J^{c}(\pi_{{\bm{\theta}}_k})+\dfrac{1}{1-\tilde\gamma}\E_{s\sim{d}_{\pi_{\bm{\theta}_k}}^{\lambda}(\cdot),a\sim\policy(\cdot|s)}
\left[
A^{\text{GAE}(\gamma,\lambda)}_{{\pi_{\bm{\theta}_k}},C}(s,a)\right]\\
\nonumber
&~~~~~~~~~~~~~~~~~~~~~~~~~+\beta_k
\sqrt{
\E_{s\sim{d}_{{\pi_{\bm{\theta}_k}}}^{\lambda}(\cdot)}\left[\text{KL}(\pi_{\bm{\theta}_k},\policy)[s]\right]}\leq b.
\end{flalign}
Until now, the particular choice of surrogate function is heuristically motivated, we show the policy and safe constraint guarantee of the proposed CUP in Theorem \ref{them-re-cost}, and its proof is shown in Appendix \ref{sec:app-them2}.
\begin{theorem}
\label{them-re-cost}
Let $\chi_k=\E_{s\sim{d}_{{\pi_{\bm{\theta}_k}}}^{\lambda}(\cdot)}\left[\emph{KL}\left(\pi_{\bm{\theta}_k},\pi_{\bm{\theta}_{k+\frac{1}{2}}}\right)[s]\right]$, if $\pi_{\bm{\theta}_k}$ and 
$\pi_{\bm{\theta}_{k+1}}$ are related to (\ref{performance-improvement})-(\ref{projection}),
then the lower bound on policy improvement, and upper bound on constraint violation are
\begin{flalign}
\nonumber
J(\pi_{\bm{\theta}_{k+1}})-J(\pi_{\bm{\theta}_{k}})\ge&-\frac{\gamma(1-\lambda)\sqrt{2\chi_k}\epsilon^{V}_{\policy}(\policyy)}{(1-\gamma)\left|1-2\gamma\lambda|\calS||\calA|\right|},\\
\nonumber
J^{c}(\pi_{\bm{\theta}_{k+1}})\leq& b+\frac{\gamma(1-\lambda)\sqrt{2\chi_k}\epsilon^{C}_{\policy}(\policyy)}{(1-\gamma)\left|1-2\gamma\lambda|\calS||\calA|\right|}.
\end{flalign}
\end{theorem}
\begin{remark}
\label{remark:Comparison-with-soda}
Let $\lambda\rightarrow0$, according to Theorem \ref{them-re-cost}, the performance and cost constraint of CUP satisfies
\begin{flalign}
\label{bound-cost-performance}
J(\pi_{\bm{\theta}_{k+1}})-J(\pi_{\bm{\theta}_{k}})&\ge-\frac{\gamma\sqrt{2\chi_k}\epsilon^{V}_{\policy}(\policyy)}{(1-\gamma)},
\\
J^{c}(\pi_{\bm{\theta}_{k+1}})&\leq b+\frac{\gamma\sqrt{2\chi_k}\epsilon^{C}_{\policy}(\policyy)}{(1-\gamma)}.
\end{flalign}
The bounds of CUP in (\ref{bound-cost-performance}) achieves at $\mathcal{O}(\frac{\gamma}{1-\gamma})$ or $\mathcal{O}(\frac{\gamma}{1-\gamma})$,
which is more tight than the bounds of CPO \citep[Proposition 1-2]{AchiamHTA17}, PCPO \citep[Theorem 1]{yang2020projection} and FOCOPS \citep{zhang2020first} where their bounds achieve at $\mathcal{O}(\frac{\gamma}{(1-\gamma)^2})$.
\end{remark}









\textbf{Practical Implementation}


Now, we present our sample-based implementation for CUP (\ref{performance-improvement})-(\ref{projection}).
Our main idea is to estimate the objective and constraints in (\ref{performance-improvement})-(\ref{projection}) with samples collected by current policy $\pi_{\bm{\theta}_k}$, then solving its optimization problem via first-order optimizer.



We denote the empirical KL-divergence with respect to $\policy$ and $\policyy$ as:
\[\hat{D}_{\text{KL}}(\policy,\policyy)=\frac{1}{T}\sum_{t=1}^{T}\text{KL}(\policy(a_t|s_t),\policyy(a_t|s_t)).\]
Let $\{(s_t,a_t,r_{t+1},c_{t+1})\}_{t=1}^{T}\sim\pi_{\bm{\theta}_k}$, we update performance improvement (\ref{performance-improvement}) step as follows,
\begin{flalign}
%\label{practical-01}
\nonumber
\pi_{{\bm{\theta}}_{k+\frac{1}{2}}}&=\arg\max_{\pi_{\bm{\theta}}\in\Pi_{\theta}}\left\{\hat{\mathcal{L}}_{\text{R}}(\policy,\pi_{{\bm{\theta}}_k})\right\}
\\
\nonumber
\hat{\mathcal{L}}_{\text{R}}(\policy,\pi_{{\bm{\theta}}_k})&=\frac{1}{T}\sum_{t=1}^{T}\dfrac{\pi_{\bm{\theta}}(a_t|s_t)}{\pi_{{\bm{\theta}}_k}(a_t|s_t)}\hat{A}_t-\alpha_k\sqrt{\hat{D}_{\text{KL}}(\pi_{{\bm{\theta}}_k},\pi_{{\bm{\theta}}})},
\end{flalign}
where $\hat{A}_t$ is an estimator of $A^{\text{GAE}(\gamma,\lambda)}_{\pi_{{\bm{\theta}}_k}}(s,a)$.
%, $\hat{D}_{\text{KL}}(\pi_{{\bm{\theta}}_k},\pi_{{\bm{\theta}}})=\frac{1}{T}\sum_{t=1}^{N}\text{KL}(\pi_{{\bm{\theta}}_k}(\cdot|s_t),\pi_{{\bm{\theta}}}(\cdot|s_t))$.


Then we update the projection step by replacing the distance function $D$ by KL-divergence, and we solve the constraint problem (\ref{projection}) by the following primal-dual approach, 
\begin{flalign}
\nonumber
%\label{practical-02}
(\pi_{{\bm{\theta}}_{k+1}},\nu_{k+1})=\arg\min_{\pi_{\bm{\theta}}\in\Pi_{\bm{\theta}}}\max_{\nu\ge0}
\left\{
\hat{\mathcal{L}}_{\text{c}}\left(\policy,\pi_{{\bm{\theta}}_k},{\bm{\theta}}_{k+\frac{1}{2}}\right)
\right\}\\
\nonumber
\hat{\mathcal{L}}_{\text{c}}\left(\policy,\pi_{{\bm{\theta}}_k},{\bm{\theta}}_{k+\frac{1}{2}}\right)=
\hat{D}_{\text{KL}}(\pi_{{\bm{\theta}}_{k+\frac{1}{2}}},\pi_{{\bm{\theta}}})
+\nu \hat{C}(\policy,\pi_{{\bm{\theta}}_k}),
\end{flalign}
where
$\hat{C}(\policy,\pi_{{\bm{\theta}}_k})=\hat{J}^{C}+\frac{1}{1-\tilde\gamma}\cdot\frac{1}{T}\sum_{t=1}^{T}\frac{\pi_{\bm{\theta}}(a_{t}|s_{t})}{\pi_{{\bm{\theta}}_k}(a_{t}|s_{t})}\hat{A}^{C}_{t}+\beta_k\sqrt{\hat{D}_{\text{KL}}(\pi_{{\bm{\theta}}_k},\pi_{{\bm{\theta}}})}-b,$ $\hat{J}^{C}$and $\hat{A}^{C}_{t}$ are estimators for cost-return and cost-advantage.

Due to the limitation of space, we present all the details of the implementation in Appendix \ref{sec-app-cpu} and Algorithm \ref{alg-app-cpu}.

==> related-work.tex <==


\section{Related Work}


This section reviews three typical ways to solve safe reinforcement learning: local policy search, Lagrangian approach, and constrained policy optimization (CPO).
We provide more comparisons and discussions in Appendix \ref{app-related-work} and Table \ref{app-table-com}.



\subsection{Local Policy Search and Lagrangian Approach}
A direct way to solve CMDP (\ref{def:problem-setting}) is to apply \emph{local policy search} \citep{kakade2002approximately,peter2008Reinforcement,2013Safepolicy} over the policy space $\Pi_{\calC}$, i.e.,
\begin{flalign}
\label{local-policy-search}
\pi_{{{\bm{\theta}}}_{k+1}}=\arg\max_{\pi_{{\bm{\theta}}}\in\Pi_{{\bm{\theta}}}}J(\pi_{{\bm{\theta}}}),~\text{s.t}.~J^{c}(\pi_{{\bm{\theta}}})\leq b,~\text{and}~D(\pi_{{\bm{\theta}}},\pi_{{{\bm{\theta}}}_{k}})<\delta,
\end{flalign}
where $\delta$ is a positive scalar, $D(\cdot,\cdot)$ is some distance measure.
For practice, the local policy search (\ref{local-policy-search}) is challenging to implement because it requires evaluation of the constraint function $c$ to determine whether a proposed point $\pi$ is feasible \citep{zhang2020first}. 
Besides, when updating policy according to samples, local policy search (\ref{local-policy-search}) requires off-policy evaluation \citep{AchiamHTA17}, which is very challenging for high-dimension control problem \citep{duan2016benchmarking,yang-ijcai2018-414,yang2020convergence}.
Thus, local policy search (\ref{local-policy-search}) looks simple, but it is impractical for high-dimension policy optimization.




The standard way to solve CMDP (\ref{def:problem-setting}) is Lagrangian approach \citep{chow2017risk} that is also known as primal-dual policy optimization \citep{chen2021primal}:
\begin{flalign}
\label{min-max-search}
(\pi_{\star},\lambda_{\star})=\arg\min_{\lambda\ge0}\max_{\policy\in\Pi_{\bm{\theta}}}
\left\{
J(\policy)-\lambda(J^{c}(\policy)-b)
\right\}.
\end{flalign}
Although extensive canonical algorithms are proposed to solve problem (\ref{min-max-search}), e.g., \citep{liang2018accelerated,tessler2019reward,paternain2019constrained,le2019batch,russel2020robust,xu2020primal,satija2020constrained,chen2021primal},
the policy updated by Lagrangian approach may be infeasible w.r.t. CMDP (\ref{def:problem-setting}).
This is hazardous in reinforcement learning when one needs to execute the intermediate policy (which may be unsafe) during training \citep{chow2018lyapunov}.

\subsection{Constrained Policy Optimization (CPO)}

Recently, \cite{AchiamHTA17} suggest to replace the cost constraint with a surrogate cost function which evaluates the constraint $J^{c}(\pi_{{\bm{\theta}}})$ according to the samples collected from the current policy $\pi_{{\bm{\theta}}_k}$. 
%Although using a surrogate function to replace the cumulative constraint cost has appeared in \citep{gabor1998multi,dalal2018safe,el2016convex}, \citep{AchiamHTA17} firstly show their algorithm guarantees for near-constraint satisfaction.
For a given policy $\pi_{{\bm{\theta}}_{k}}$, CPO \citep{AchiamHTA17} updates new policy $\pi_{{\bm{\theta}}_{k+1}}$ as follows:
%\footnote
%{
%The objective presented by \cite{AchiamHTA17} is $\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),{\color{red}{a\sim\pi_{{\bm{\theta}}}(\cdot|s)}}}[A_{\pi_{{\bm{\theta}}_k}}(s,a)]$, which is same as the presentation in Eq.(\ref{cpo-objective}) since 
%$\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),{\color{blue}{a\sim\pi_{{\bm{\theta}}_k}(\cdot|s)}}}[\frac{\pi_{{\bm{\theta}}}(a|s)}{\pi_{{\bm{\theta}}_k}(a|s)}A_{\pi_{{\bm{\theta}}_k}}(s,a)]=\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),{\color{red}{a\sim\pi_{{\bm{\theta}}}(\cdot|s)}}}[A_{\pi_{{\bm{\theta}}_k}}(s,a)]$.
%}
\begin{flalign}
\label{cpo-objective}
&\pi_{{\bm{\theta}}_{k+1}}=\arg\max_{\pi_{{\bm{\theta}}}\in\Pi_{{\bm{\theta}}}}~~~~\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),a\sim\pi_{{\bm{\theta}}}(\cdot|s)}\left[A_{\pi_{{\bm{\theta}}_k}}(s,a)\right]\\
\label{cost-constraint}
&~~~~~~~~\text{s.t.}~~J^{c}(\pi_{{\bm{\theta}}_k})+\frac{1}{1-\gamma}\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot),a\sim\pi_{{\bm{\theta}}}(\cdot|s)}\left[A^{c}_{\pi_{{\bm{\theta}}_k}}(s,a)\right]\leq b,\\
\label{trust-region}
&~~~~~~~~\bar{D}_{\text{KL}}(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_k})=\E_{s\sim d^{\rho_0}_{\pi_{{\bm{\theta}}_k}}(\cdot)}[\text{KL}(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_k})[s]]\leq\delta.
\end{flalign}
Existing recent works (e.g., \citep{AchiamHTA17,vuong2019supervised,yang2020projection,hanreinforcementl2020,ijcai2020-632,bharadhwaj2021conservative}) try to find some convex approximations to replace the term $A_{\pi_{{\bm{\theta}}_k}}(s,a)$ and $\bar{D}_{\text{KL}}(\pi_{{\bm{\theta}}},\pi_{{\bm{\theta}}_k})$ Eq.(\ref{cpo-objective})-(\ref{trust-region}).
%Concretely, according to (\ref{performance-difference-2002}), \cite{AchiamHTA17} suggest to use first-order Taylor expansion to replace (\ref{cpo-objective})-(\ref{cost-constraint}), use second-oder approximation to replace (\ref{trust-region}).
Such first-order and second-order approximations turn a non-convex problem (\ref{cpo-objective})-(\ref{trust-region}) to be a convex problem, 
it seems to make a simple solution, but this approach results in many error sources and troubles in practice.
Firstly, it still lacks a theory analysis to show the difference between the non-convex problem (\ref{cpo-objective})-(\ref{trust-region}) and its convex approximation.
Policy optimization is a typical non-convex problem \citep{yang2021sample}; its convex approximation may introduce some error for its original issue.
Secondly, CPO updates parameters according to conjugate gradient \citep{suli2003introduction}, and its solution involves the inverse Fisher information matrix,
which requires expensive computation for each update.
Later, \cite{yang2020projection} propose projected-based constrained policy optimization (PCPO) that also uses second-order approximation, which also results in an expensive computation.


Instead of using a convex approximation for the objective function, the proposed CUP algorithm improves CPO and PCPO at least two aspects.
Firstly, the CUP directly optimizes the surrogate objective function via the first-order method, and it does not depend on any convex approximation.
Thus, the CUP effectively avoids the expensive computation for the inverse Fisher information matrix.
Secondly, CUP extends the surrogate objective function to GAE. Although \cite{zhang2020first} has used the GAE technique in experiments, to the best of our knowledge, it still lacks a rigorous theoretical analysis involved GAE before we propose CUP.






